On the Dirichlet Problem for First Order Hyperbolic PDEs on Bounded Domains with Mere Inflow Boundary: Part II Quasi-Linear Equations

We study the Dirichlet problem for first order hyperbolic quasi-linear functional PDEs on a simply connected bounded domain of $\R^2$, where the domain has an interior outflow set and a mere inflow boundary. While the question of existence of a solution has already been answered in its predecessor, the present paper discusses the uniqueness and continuous dependence on the coefficients of the PDE. Under the assumption that the functional dependence is causal, we are able to derive a contraction principle which is the key to proof uniqueness and continuous dependence. Such a causal functional dependence appears, e.g., in transport based image inpainting.

==> macros.tex <==
%%
% at "@" und "!" als letter
%% 
\expandafter\edef\csname @catcode\endcsname{\the\catcode`\@}
\expandafter\edef\csname !catcode\endcsname{\the\catcode`\!}
\catcode`\@11
\catcode`\!11

%%%% skips
\smallskipamount=3pt plus 0.5pt minus 0.5pt
\medskipamount=6pt plus 1pt minus 1pt
\bigskipamount=12pt plus 2pt minus 2pt

%%% Tabellen
\renewcommand{\arraystretch}{1.5}

%%% Mengen
\def\A{{\mathcal{A}}}                 %% generische sigma-Algebra
\def\B{{\mathcal{B}}}                 %% Borel-sigma-Algebra
\def\Sk{{\mathcal{S}}} 		%% Skelett
\def\N{{\mathbb{N}}}                  %% natürliche Zahlen
\def\Z{{\mathbb{Z}}}                  %% ganze Zahlen
\def\R{{\mathbb{R}}}                  %% reellen Zahlen
\def\1{{\mathbb{1}}}			%% charakteristische Funktion
\def\Rinfty{\overline{\mathbb{R}} }         %% reellen Zahlen mit +infty und -infty


% meine Funktionenmengen
\def\FD{{\mathcal{F}}}                %% Functional domain general
\def\FR{{\mathcal{G}}}                %% Functional range general
\def\FF{{\mathfrak{F}}}                 %% Functional domain in L^1
\def\FX{{\mathfrak{X}}}                %%  Functional domain in BV
\def\FB{{\mathfrak{B}}}                %%  Randfunktionen aus BV  
                

%%% Parameter
\def\const{{\mathrm{const}}}          %% irgendeine Konstance

%%% Funktionenräume 
\def\C{C}                                      %% stetige Funktionen
\def\L{L}                                         %% Lebesgue intbare Funktionen
\def\Lloc{L_{\mathrm{loc}}}           %% lokal Lebesgue intbare Funktionen
\def\W{W}                                          %% Sobolev Raum
\def\BV{{\mathit{BV}}}                %% Funktionen beschr. Variation
\def\SBV{{\mathit{SBV}}}              %% spez. Funktionen beschr. Variation
\def\PT{{\mathit{P}}}                %% periodische Testfunktionen

%%% Maße
\def\Hm{{\mathcal{H}}}                %% Hausdorff-Maß
\def\Lm{{\mathcal{L}}}                %% Lebesgue-Maß
\def\Mloc{{\mathcal{M}_{\mathrm{loc}}}}%% vektorwertige Radon-Maße
\def\M{{\mathcal{M}}}                 %% endliche Radon-Maße

%% Verweis auf Gleichung
\def\refEq#1{(\ref{#1})}

%% Intervall
\def\IV#1#2,#3#4{\left#1#2,#3\right#4}
\def\usIV#1#2;#3#4{\mathopen{#1}#2;#3\mathclose{#4}}

%% Skalarprodukt / Norm
\def\SP#1#2,#3#4{\left#1#2,#3\right#4}
\def\Norm#1#2{\Vert#1\Vert_{#2}}                                   %% Norm
\def\sNorm#1#2{\left\Vert#1\right\Vert_{#2}}                 %% sNorm: norm mit left und right Skalierung
\def\genNorm#1{\Vert#1\Vert}                                          %% generische Norm

%% Operatoren
\def\arclength{\mathop{\operator@font arclength}}                       %% Bogenlänge
\let\bd\partial                                                                                          %% Rand, boundary
\let\pd\partial                                                                                          %% partial derivative
\let\cl\overline                                                                                         %% Abschluss closure
\def\div{\mathop{\operator@font div}}                                             %% Divergenz
\DeclareMathOperator{\dist}{dist}                              %% distance
\def\liminf{\mathop{\smash{\operator@font lim\,inf}}}        % liminf
\def\limsup{\mathop{\smash{\operator@font lim\,sup}}}        % limsup
\def\supp{\mathop{\smash{\operator@font supp}}}          % support
\def\O{\mathcal{O}}                                          % Landau
\def\o{{o}}                                                          % Landau klein
\def\Var{\mathop{\operator@font Var}}                        % Variation
\def\trace{\mathop{\operator@font trace}}                        % spur
\DeclareMathOperator{\sgn}{sgn}                                % signum
\DeclareMathOperator{\lingen}{span}                                % span
\def\inner#1{\mathring{#1}} 
\def\diam{\mathop{\operator@font diam}}                         %% Diameter

%%% binäre Operatoren
\def\longrightharpoonup{%                                    % long-Variante von rightharpoonup
  \relbar\joinrel\rightharpoonup
}
\let\wo\backslash                                            %% ohne
\let\nb\sim                                                  %% Nachbarschaft
\def\rto{\,\hbox{\vrule height7pt width0.5pt depth0pt        %% Restriktion
  \vrule height0.5pt width5pt depth0pt}\,}
\def\cc{\mathbin{\mathord{\subset}\!\mathord{\subset}}}        %% compact subset
\let\asymp\sim                                               %% asymptot. Verh.
\def\symdiff{\mathbin{\Delta}}                               %% symmetr. Diff.
\let\gdw\Leftrightarrow                                      %% genau dann wenn
\def\strongto{%                                              %% starke Konvergenz
  \@ifnextchar[\@strongto{\@strongto[]}}
\def\@strongto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \to
  \else
  \mathrel{\mathop{\longrightarrow}\limits_{\scriptstyle#1}}%
  \fi
}
\def\weakto{%                                                % schwache Konvergenz
  \@ifnextchar[\@weakto{\@weakto[]}}
\def\@weakto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \rightharpoonup
  \else
  \mathrel{\mathop{\longrightharpoonup}\limits_{\scriptstyle#1}}%
  \fi
}
\def\weaksto{%                                                % schwache* Konvergenz
  \@ifnextchar[\@weaksto{\@weaksto[]}}
\def\@weaksto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \mathrel{\mathop{\rightharpoonup}\limits^{\scriptstyle*}}%
  \else
  \mathrel{\mathop{\longrightharpoonup}\limits^{\scriptstyle*}_{\scriptstyle#1}}%
  \fi
}
\let\symdiff\Delta                                            % symmetrische Differenz
\def\dotarg{\mathord{\, .\,}}                              % beliebiges Argument mit Punkt


%%
% Theoreme und Environments
%%


\newtheorem{theo}{Theorem}[section]
\newtheorem{lem}[theo]{Lemma}%[chapter]
\newtheorem{cor}[theo]{Corollary}%[chapter]
\newtheorem{prop}[theo]{Proposition}%[chapter]
\newtheorem{defi}[theo]{Definition}%[chapter]
\newtheorem{req}[theo]{Requirement}%[chapter]
\newtheorem{prob}[theo]{Problem}%[chapter]
\newtheorem{rem}[theo]{Remark}%[chapter]

%% Beweis:
%% Umbruch danach nicht unerwünscht
%\let\orig@end@proof\endproof
%\def\endproof{\orig@end@proof\penalty-500\relax}

%% Davor hat auch niemand was dagegen
%\let\orig@proof\proof
%\def\proof{\penalty-500 \orig@proof}


%% kein Absatz Einzug
%\parindent=0pt

%% dafür aber etwas Parskip zur Abtrennung verschiedener Absätze
%\parskip=3pt plus1.5pt minus1pt

%% die Ränder
\evensidemargin=2cm %54pt
\oddsidemargin=2cm %54pt

%\advance\evensidemargin -2.5mm
%\advance\oddsidemargin -2.5mm

%% marks für Headline
%\def\chaptermark#1{%
%  \markboth {%
%    \ifnum \c@secnumdepth >\m@ne
%      \if@mainmatter
%        \@chapapp\ \thechapter\enskip%
%      \fi
%    \fi
%    #1}{}}%
%\def\sectionmark#1{%
%  \markright {%
%    \ifnum \c@secnumdepth >\z@
%      \thesection\enskip%
%    \fi
%    #1}}

\endinput

